Geometric Flow of Bubbles

In this work we derive a class of geometric flow equations for metric-scalar systems. Thereafter, we construct them from some general string frame action by performing volume-preserving fields variations and writing down the associated gradient flow equations. Then, we consider some specific realisations of the above procedure, applying the flow equations to non-trivial scalar bubble and metric bubble solutions, studying the subsequent flow behaviour.

==> BAckup.tex <==
\subsection{Geometric Flow from an Action}
In the following discussion, it is shown how geometric flow equations can be straightforwardly induced from the action
\begin{equation}
    S=\int\diff^{D}x\sqrt{\tilde{g}}\left[\tilde{R}+\frac{1}{2}\left(\nabla f\right)^{2}-\sum_{n=2}^{+\infty}\frac{g_{n}}{n!}f^{n}\right]\ .
\end{equation}
of a $D$-dimensional metric-scalar $\left(\tilde{g},f\right)$ system. In order to do so, we construct an appropriate entropy functional of the form \eqref{funk} by rescaling both $\tilde{g}_{\mu\nu}$ and $f$, so that the volume element takes the correct
\begin{equation}
    \sqrt{g}e^{-\phi}
\end{equation}
form and the general expression \eqref{geneq} for the flow equations can be straightforwardly applied, with $\phi$ being the rescaled scalar. Furthermore, in order to make connection to Perelman's entropy functional, we exploit our rescaling so that the $\alpha$ prefactor in front of $\left(\nabla \phi\right)^2$ is just one. Thus, we define:
\begin{equation}
    \tilde{g}_{\mu\nu}\equiv e^{2\varphi}g_{\mu\nu},\quad f\equiv\gamma\phi\ .
\end{equation}
By plugging these definitions into the metric, we have:
\begin{equation}
\begin{split}
     S=\int\diff^{D}x\sqrt{g}e^{\left(D-2\right)\varphi}\biggl[&R-2(D-1)\Delta\varphi-(D-2)(D-1)\left(\nabla\varphi\right)^2+\\
     &+\frac{\gamma^{2}}{2}\left(\nabla \phi\right)^{2}-e^{2\varphi}\sum_{n=2}^{+\infty}\frac{\gamma^{n}g_{n}}{n!}\phi^{n}\biggr]\ .
\end{split}
\end{equation}
For the volume element to take the appropriate form, we take:
\begin{equation}
    \varphi\equiv\frac{1}{2-D}\phi\ .
\end{equation}
Therefore, we obtain:
\begin{equation}
\begin{split}
     S=\int\diff^{D}x\sqrt{g}e^{-\phi}\biggl[&R+2\frac{D-1}{D-2}\Delta \phi+\left(\frac{\gamma^{2}}{2}-\frac{D-1}{D-2}\right)\left(\nabla \phi\right)^2+\\
     &-\exp{\left(\frac{2\phi}{2-D}\right)}\sum_{n=2}^{+\infty}\frac{\gamma^{n}g_{n}}{n!}\phi^{n}\biggr]\ .
\end{split}
\end{equation}
In order to connect ourselves to Perelman's entropy functional, we take:
\begin{equation}
    \frac{\gamma^{2}}{2}-\frac{D-1}{D-2}=1\Longrightarrow\gamma=\sqrt{\frac{4D-6}{D-2}}\ .
\end{equation}
Hence, we are left with:
\begin{equation}
    \begin{split}
     S=\int\diff^{D}x\sqrt{g}e^{-\phi}\biggl[&R+2\frac{D-1}{D-2}\Delta \phi+\left(\nabla \phi\right)^2+\\
     &-\exp{\left(\frac{2\phi}{2-D}\right)}\sum_{n=2}^{+\infty}\frac{g_{n}}{n!}\left(\frac{4D-6}{D-2}\right)^{n/2}\phi^{n}\biggr]\ .
\end{split}
\end{equation}
The last term still needs to be expressed in a more treatable way. Thus,we define
\begin{equation}
    p\equiv\frac{2}{2-D},\quad q_{n}\equiv\frac{g_{n}}{n!}\left(\frac{4D-6}{D-2}\right)^{n/2}
\end{equation}
and observe that:
\begin{equation}
    \begin{split}
        \exp{\left(p\phi\right)}\sum_{n=2}^{+\infty}q_{n}\phi^{n}=&\sum_{k=0}^{+\infty}\frac{p^{k}}{k!}\phi^{k}\cdot\sum_{n=0}^{+\infty}q_{n+2}\phi^{n+2}\ .
    \end{split}
\end{equation}
By defining
\begin{equation}
    p_{k}\equiv\frac{p^{k}}{k!}\ ,
\end{equation}
we further have:
\begin{equation}
    \begin{split}
        \exp{\left(p\phi\right)}\sum_{n=2}^{+\infty}q_{n}\phi^{n}=&\sum_{k=0}^{+\infty}p_{k}\phi^{k}\cdot\sum_{n=0}^{+\infty}q_{n+2}\phi^{n+2}=\\
        =&\sum_{k=0}^{+\infty}\sum_{n=0}^{k}p_{k-n}\phi^{k-n}q_{n+2}\phi^{n+2}=\\
        =&\sum_{k=0}^{+\infty}\phi^{k+2}\sum_{n=0}^{k}p_{k-n}q_{n+2}=\\
        =&\sum_{k=0}^{+\infty}\phi^{k+2}\sum_{n=0}^{k}\frac{g_{n+2}}{\left(k-n\right)!\left(n+2\right)!}\left(\frac{2}{2-D}\right)^{k-n}\left(\frac{4D-6}{D-2}\right)^{n/2+1}=\\
        =&\sum_{k=2}^{+\infty}\phi^{k}\sum_{n=0}^{k-2}\frac{g_{n+2}}{\left(k-2-n\right)!\left(n+2\right)!}\left(\frac{2}{2-D}\right)^{k-2-n}\left(\frac{4D-6}{D-2}\right)^{n/2+1}\ .
    \end{split}
\end{equation}
Therefore, as we define
\begin{equation}
    s_{\ k}^{(D)}\equiv\sum_{n=0}^{k-2}\frac{g_{n+2}}{\left(k-2-n\right)!\left(n+2\right)!}\left(\frac{2}{2-D}\right)^{k-2-n}\left(\frac{4D-6}{D-2}\right)^{n/2+1}
\end{equation}
for $k>1$, we get the following form of the action:
\begin{equation}
     S=\int\diff^{D}x\sqrt{g}e^{-\phi}\biggl[R+2\frac{D-1}{D-2}\Delta \phi+\left(\nabla \phi\right)^2-\sum_{n=2}^{+\infty}s_{\ n}^{(D)}\phi^{n}\biggr]\ .
\end{equation}
Hence, we precisely have a functional as the one described in \eqref{funk}, with:
\begin{equation}
    \alpha=1,\quad\gamma=2\frac{D-1}{D-2},\quad\beta_{n}=-s_{\ n}^{(D)}\ .
\end{equation}
The associated flow equations are:
\begin{equation}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}-g_{\mu\nu}\sum_{n=2}^{+\infty}ns_{\ n}^{(D)}\phi^{n-1}+4\frac{D-1}{D-2}\nabla_{\mu}\phi\nabla_{\nu}\phi-2\frac{5D-6}{D-2}\nabla_{\nu}\nabla_{\mu}\phi+\\
        &-2\frac{D-1}{D-2}g_{\mu\nu}\nabla^{2}\phi+2\frac{D-1}{D-2}g_{\mu\nu}\left(\nabla \phi\right)^2+\mathcal{L}_{\xi}g_{\mu\nu}\ ,\\
        \frac{\de \phi}{\de\lambda}=&-R-\frac{D}{2}\sum_{n=2}^{+\infty}ns_{\ n}^{(D)} \phi^{n-1}+\frac{\left(D-1\right)\left(D+2\right)}{D-2}\left(\nabla \phi\right)^{2}+\\
        &-\frac{D^{2}+4D-6}{D-2}\nabla^{2} \phi+\mathcal{L}_{\xi} \phi\ .
    \end{split}
\end{equation}
Therefore, we have derived a general expression for the geometric flow equations induced by the $D$-dimensional action for a metric-scalar system with arbitrary polynomial self-interaction terms, by defining the entropy functional as its string-frame version. 
\subsection{Massive Perelman's Flow}
We now focus on the specific example of a massive scalar field with no other coupling, on a space-time background admitting a cosmological constant. Namely, we take:
\begin{equation}
    \left(g_{0},g_{1},g_{2},g_{3},\dots\right)\equiv\left(\Lambda,0,m^{2},0,\dots\right)
\end{equation}
Therefore, we get:
\begin{equation}
    s_{\ k}^{(D)}=\frac{m^{2}}{\left(k-2\right)!}\frac{2D-3}{D-2}\left(\frac{2}{2-D}\right)^{k-2}\ .
\end{equation}
Furthermore, we assume the scalar to take a constant value $f$ and the metric to be that of an Einstein manifold, with:
\begin{equation}
    R_{\mu\nu}=\frac{R}{D} g_{\mu\nu}\ .
\end{equation}
Therefore, the flow equations reduce to:
\begin{equation}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}\sum_{n=2}^{+\infty}ns_{\ n}^{(D)}f^{n-1}+\mathcal{L}_{\xi}g_{\mu\nu}\ ,\\
        \frac{\de f}{\de\lambda}=&-R-\frac{D}{2}\sum_{n=2}^{+\infty}ns_{\ n}^{(D)} f^{n-1}+\mathcal{L}_{\xi} f\ .
    \end{split}
\end{equation}
It can be derived that:
\begin{equation}
    \begin{split}
        \sum_{k=2}^{+\infty}ks_{\ k}^{(D)}f^{k-1}=&        \sum_{k=2}^{+\infty}k\frac{m^{2}}{\left(k-2\right)!}\frac{2D-3}{D-2}\left(\frac{2}{2-D}\right)^{k-2}f^{k-1}=\\
        =&\frac{2D-3}{D-2}m^{2}f\sum_{k=0}^{+\infty}\frac{k+2}{k!}\left(\frac{2}{2-D}\right)^{k}f^{k}=\\
        =&\frac{2D-3}{D-2}m^{2}f\left(2+f\frac{\de}{\de f}\right)\exp{\left(\frac{2f}{2-D}\right)}\equiv F_{f}\ .
    \end{split}
\end{equation}
Thus, by neglecting the diffeomorphisms, we have:
\begin{equation}
        \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}F_{f}\ ,\\
        \frac{\de f}{\de\lambda}=&-R-\frac{D}{2}F_{f}\ .
    \end{split}
\end{equation}
By recasting the first equation in terms of the scalar curvature, we have:
\begin{equation}
\frac{\de R}{\de\lambda}=\frac{2R}{D}\left(R+\frac{D}{2}F_{f}\right)\ .
\end{equation}
Hence, by defining
\begin{equation}
    \mathcal{A}\left(R,f\right)\equiv R+\frac{D}{2}F_{f}\ ,
\end{equation}
we can solve for:
\begin{equation}
        \begin{split}
            \frac{\de R}{\de\lambda}=&\frac{2R}{D}\mathcal{A}\left(R,f\right)\ ,\\
        \frac{\de f}{\de\lambda}=&-\mathcal{A}\left(R,f\right)\ .
    \end{split}
\end{equation}
Since $m$ is the only scale present in the following discussion, we can set it to $1$ without loss of generality. 
\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Ff.png}
    \caption{Plot of $F_{f}$ with respect to $f$, at $m=1$, for different values of the dimension $D$, taken between $3$ and $8$.\\}
    \includegraphics[width=0.6\linewidth]{Gr.png}
    \caption{The blue region corresponds to $\mathcal{A}>0$, with $D=4$. The arrows correspond to the flow direction.}
\end{figure}
From the above picture it is clear that the $\mathcal{A}=0$ line, separating the blue and the white regions, can either be a stable or an unstable fixed point. In particular, fixed points can only exist for $R>R_{0}$, for some negative $R_{0}$. Indeed, fixed points form two branches:
\begin{itemize}
    \item The higher branch, with bigger values of $f$, is unstable;
    \item The lower branch, with smaller values of $f$, is stable.
\end{itemize}
In order to better analyse the system, we perform a diffeomorphism
\begin{equation}
        \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}F_{f}+\mathcal{L}_{\chi}g_{\mu\nu}=\\
        =&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}F_{f}+\nabla_{\mu}\chi_{\nu}+\nabla_{\nu}\chi_{\mu}\ ,\\
        \frac{\de f}{\de\lambda}=&-R-\frac{D}{2}F_{f}+\mathcal{L}_{\chi}f=\\
        =&-R-\frac{D}{2}F_{f}+\chi^{\mu}\de_{\mu}f\ ,
    \end{split}
\end{equation}
sourced by a vector field $\chi^{\mu}$. In particular, we impose:
\begin{equation}
    \nabla_{\mu}\chi_{\nu}+\nabla_{\nu}\chi_{\mu}=g_{\mu\nu}F_{f}\ .
\end{equation}
By contracting with the inverse metric, we get:
\begin{equation}
    \nabla_{\mu}\chi^{\mu}=\frac{D}{2}F_{f}\ .
\end{equation}
Expanding the two sides, we see that $\chi$ depends on the flow-dependent metric and scalar in a highly non-trivial way:
\begin{equation}
    \partial_{\mu}\chi^{\mu}+\frac{1}{2}g^{\mu\alpha}\chi^{\nu}\partial_{\nu}g_{\alpha\mu}=\frac{D}{2}F_{f}
\end{equation}
By defining
\begin{equation}
    \begin{split}
    A_{\nu}&\equiv -\frac{1}{2}g^{\mu\alpha}\partial_{\nu}g_{\alpha\mu}\ ,\\
        B&\equiv \frac{D}{2}F_{f}\ ,
    \end{split}
\end{equation}
we get:
\begin{equation}
    \partial_{\mu}\chi^{\mu}\left(x\right)=A_{\mu}\left(x\right)\chi^{\mu}\left(x\right)+B\left(x\right)\ .
\end{equation}
We make, in spherical coordinates
\begin{equation}
    g=diag\left(-G(r),G(r)^{-1},r^{2},r^{2}\sin^{2}{\vartheta}\right)\ ,
\end{equation}
the following ansatz:
\begin{equation}
    \chi^{\mu}=\delta^{\mu}_{r}\rho(r)\ .
\end{equation}
Hence, we get
\begin{equation}
    \rho'(r)=\frac{4}{r}\rho(r)+B(r)\ ,
\end{equation}
which can be solved as:
\begin{equation}
    \rho(r)=r^{4}\int^{r}_{0}\frac{B\left(\xi\right)}{\xi^{4}}\diff\xi=r^{4}\frac{D}{2}\int^{r}_{0}\frac{F_{f}\left(\xi\right)}{\xi^{4}}\diff\xi\ .
\end{equation}
Therefore, under the diffeomorphism we get:
\begin{equation}
           \begin{split}
        \frac{\de R}{\de\lambda}=&\frac{2R^{2}}{D}\ ,\\
        \frac{\de f}{\de\lambda}=&-R-\frac{D}{2}F_{f}+\rho(r)\de_{r}f\ .
    \end{split} 
\end{equation}
We have:
\begin{equation}
    R\left(\lambda\right)=\frac{DR_{0}}{D-2R_{0}\lambda}\ .
\end{equation}
Hence, we only have to solve for:
\begin{equation}
\begin{split}
    \frac{\de f}{\de\lambda}=&\frac{DR_{0}}{2R_{0}\lambda-D}-\frac{D}{2}F_{f}+\frac{\de f}{\de r}\frac{r^{4}D}{2}\int^{r}_{0}\frac{F_{f}\left(\xi\right)}{\xi^{4}}\diff\xi=\\
    =&\frac{DR_{0}}{2R_{0}\lambda-D}-\frac{D}{2}\frac{2D-3}{D-2}m^{2}f\left(2+f\frac{\de}{\de f}\right)\exp{\left(\frac{2f}{2-D}\right)}+\\
    &+\frac{\de f}{\de r}\frac{r^{4}D}{2}\int^{r}_{0}\frac{2D-3}{D-2}m^{2}f\left(2+f\frac{\de}{\de f}\right)\exp{\left(\frac{2f}{2-D}\right)}\xi^{-4}\diff\xi
    \end{split}
\end{equation}
For $D=4$ and $m=1$, with $f$ constant, we get:
\begin{equation}
\begin{split}
    \frac{\de f}{\de\lambda}=&\frac{2R_{0}}{R_{0}\lambda-2}+5f\bigl(f-2\bigr)e^{-f}\ .
    \end{split}
\end{equation}
\subsubsection{Definition of the fields}
In the following discussion, we assume to work with a spherically symmetric, $4$-dimensional, vacuum solution to Einstein field equations with cosmological constant $\Lambda$ and with a spherically symmetric dilaton $f$. Therefore, we have:
\begin{equation}\label{invar}
    R_{\mu\nu}=\Lambda g_{\mu\nu}\ ,\qquad R=4\Lambda\ .
\end{equation}
Starting from \eqref{form2}, the flow equation for the metric can be recasted in terms of the scalar curvature as follows:
\begin{equation}\label{curv1}
    \Dot{R}=\Delta R+2R^{\mu\nu}R_{\mu\nu}\ .
\end{equation}
Starting from \eqref{form1}, instead, we have:
\begin{equation}\label{curv2}
\begin{split}
    \Dot{R}=&\Delta R+2R^{\mu\nu}R_{\mu\nu}+2R^{\mu\nu}\nabla_{\mu}\nabla_{\nu}f+2\nabla_{\mu}\left[\nabla^{\mu},\nabla^{\nu}\right]\nabla_{\nu}f\\
    =&\Delta R+2R^{\mu\nu}R_{\mu\nu}+2R^{\mu\nu}\nabla_{\mu}\nabla_{\nu}f-2R_{\mu\nu}\nabla^{\nu}\nabla^{\mu}f=\\
    =&\Delta R+2R^{\mu\nu}R_{\mu\nu}\ .
\end{split}
\end{equation}
The fact that the two sets of equations provide us with the same evolution for $R$ is consistent with them being related via a diffeomorphism.
In spherical coordinates, the metric tensor, for both de Sitter $\left(\Lambda>0\right)$ and Anti-de Sitter $\left(\Lambda<0\right)$, takes the form:
\begin{equation}\label{spacetime}
    \ds^{2}=-\left(1-\frac{\Lambda r^2}{3}\right)\dt^2+\left(1-\frac{\Lambda r^2}{3}\right)^{-1}\diff r^2+r^2\diff\theta^{2}+r^2\sin^{2}{\theta}\diff\phi^2\ .
\end{equation}
In this setting, we have that solutions with $\mathcal{F}=0$ must satisfy:
\begin{equation}
\begin{split}
    f(r)=&\int\diff r\sqrt{-Rg_{rr}}=2\int\diff r\sqrt{\frac{\Lambda^{2}r^2}{3}-\Lambda}=\\ 
    =&f_{0}+r\sqrt{\frac{\Lambda^{2}r^2}{3}-\Lambda}-\sqrt{3}\log{\left[\Lambda r+\sqrt{\Lambda^{2}r^2-3\Lambda}\right]}\ .
\end{split}
\end{equation}
The above solution $f(r)$ is only well-defined in $\R$ for $r^2\geq 3/\Lambda$. When $\Lambda\leq 0$, this is trivially solved for any value of $r$. When $r^2<3/\Lambda$, possible for $\Lambda>0$, $f$ is only defined if allowed to take imaginary values. From a physical perspective, this can be interpreted as a non-zero axion contribution, only appearing in a sphere with no dilaton around the origin. Nevertheless, we do not work, here, with this kind of $f$: instead, we focus on dilatonic bubbles as the ones described in \eqref{dilaton}.\\

==> Flowing.tex <==
\subsection{Flowing $m$}
In the following discussion, we instead force \textit{both} $R$ and $\varphi$ to be \textit{on-shell}. Namely, we turn the flow into a flow for $\lambda$ and $m$. The equations can explicitly be written down as
\begin{equation}
    \begin{split}
        \frac{\diff\lambda}{\diff\mu}&=-\lambda^2\cdot K\left(m\right)\ ,\\
        \frac{\diff m}{\diff\mu}&=-2\lambda\cdot K\left(m\right)\ ,
    \end{split}
\end{equation}
where a constant $15/16$ was re-absorbed in the flow parameter and the function $K(m)$ is obtained from $G(-m)$ by making $m$ a variable in the whole expression as
\begin{equation}
    K\left(m\right)\equiv 1-\frac{15}{32}(-m)^{m-1}\sum_{l=0}^{\infty}(-m)^lc_{\ l}^{m}\ ,
\end{equation}
with:
\begin{equation}
    c_{\ l}^{m}\equiv\left(m+l\right)\frac{\left(-1\right)^l}{l!}\left(1-\frac{l\sqrt{5}}{m+1}\right)\frac{2\sqrt{5^m}}{\Gamma\left(m+1\right)}\ .
\end{equation}
As in the previous discussion, an approximate general plot is provided.
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{PlotsreamA.png}
    \caption{Plot of the vector field tangent to the flow, given generic initial conditions. In the above, the vertical axis corresponds to $m$ while the horizontal one to $\lambda$.}
\end{figure}
As can be clearly observed, the flow reaches a \textit{fixed point} with $\lambda$ smaller than $1$ and $m$ smaller than $4$.
\newpage

==> NEW.tex <==
\section{Bubble of Nothing}
According to the \textit{Cobordism Conjecture} \cite{McNamara:2019rup}, any consistent low energy quantum gravity vacuum must be cobordant to the empty set. Namely, it must admit a finite energy boundary domain wall. Nucleation of \textit{bubbles of nothing} is thus thermodynamically allowed and accessible via quantum tunnelling. In the following discussion, we will construct some toy models of such solutions and study their flow behaviour.
\subsection{Bubble in Minkowski}
Let's consider a $D$-dimensional non-compact manifold with trivial topology, endowed with Minkowski metric and global spherical coordinates. Now, let's \textit{cut} the radial coordinate at a minimal cut-off $a$, changing the topology and introducing a finite bubble of nothing at the centre of our manifold. Now, let $b>a$ define the region $\left[a,b\right]$ where the boundary domain wall is defined. Therefore, our spherically symmetric and static metric takes the form
\begin{equation}
    g_{\mu\nu}\equiv F\left(r\right)\eta_{\mu\nu}\ ,
\end{equation}
where 
\begin{equation}
    F:\left[a,+\infty\right]\longrightarrow\R
\end{equation}
is equal to $1$ for $r\geq b$ and defined as
\begin{equation}
    F\left(r\right)\equiv\frac{1}{2}\left[1+\tanh{\frac{c\left(2r-b-a\right)}{2\left(b-r\right)\left(r-a\right)}}\right]
\end{equation}
for $r\in\left[a,b\right]$, where $c$ controls the steepness of the transition. Therefore, our metric is fully characterised by the three parameters $a$, $b$ and $c$, which set the size of the bubble of nothing, the size of the defect an the wall steepness, respectively.
\section{Normalised Flow of Einstein Bubbles}
In the following section, we consider space-time kinematical states with cosmological constant bubbles. According to the Swampland Cobordism Conjecture \cite{McNamara:2019rup}, two low energy space-time configurations that admit an ultraviolet completion to quantum gravity should allow for a finite energy domain wall connecting them. From the perspective of the Swampland Distance conjecture, this means that deforming one of the two solutions in order to include a bubble in which the other is realised should correspond to a finite-distance path in the moduli space. It must be stressed that the above statement doesn't imply that \textit{any} path in the moduli space between the two must have a finite length: via including short-scale oscillations, we can trivially make any path infinitely long.
The claim is that there must be \textit{at least} one finite path connecting them. 
\subsection{Constructing a Solution}
Let $\Lambda_1$ and $\Lambda_2$ be two \textit{negative} values of the cosmological constant, corresponding to anti de Sitter solutions which are taken to belong to the landscape. Let $\Lambda_1$ be our \textit{background} value, in which a bubble characterised by $\Lambda_2$ will be supposed to appear. The most reasonable choice for a metric flow equation is the following, for which Einstein manifolds are fixed points:
\begin{equation}
    \frac{\de g_{\mu\nu}}{\de\lambda}=\frac{R}{D}g_{\mu\nu}-R_{\mu\nu}\ .
\end{equation}
\subsection{Small perturbations}
Let $e_{\mu\nu}$ be a $D$-dimensional Einstein manifold metric with cosmological constant $\Lambda$ and let $\varepsilon h_{\mu\nu}$ be a small perturbation thereof. Therefore, we have:
\begin{equation}
    g_{\mu\nu}=e_{\mu\nu}+\varepsilon h_{\mu\nu}\ .
\end{equation}
Considering the first order expression for Ricci tensor, we get:
\begin{equation}
    R_{\mu\nu}\left[g\right]\approx R_{\mu\nu}\left[e\right]+\varepsilon\frac{\delta R_{\mu\nu}}{\delta g_{\alpha\beta}}\left[e\right]h_{\alpha\beta}=\frac{2\Lambda}{D-2}\left(e_{\mu\nu}+2\varepsilon h_{\mu\nu}\right)\ .
\end{equation}
Hence, we obtain
\begin{equation}
    R\left[g\right]\approx\frac{2\Lambda}{D-2}\left(e_{\mu\nu}+2\varepsilon h_{\mu\nu}\right)\left(e^{\mu\nu}-\varepsilon h^{\mu\nu}\right)\approx\frac{2\Lambda}{D-2}\left(D+\varepsilon h\right)\ ,
\end{equation}
where $h\equiv h_{\mu\nu}e^{\mu\nu}$. By plugging the above expressions into the flow equations and solving them order-by-order in $\varepsilon$, we get that $e_{\mu\nu}$ (and hence $\Lambda$) is fixed and:
\begin{equation}
    \frac{\de h_{\mu\nu}}{\de\lambda}\approx\frac{2\Lambda}{D\left(D-2\right)}\left(he_{\mu\nu}-Dh_{\mu\nu}\right)\ .
\end{equation}
By defining
\begin{equation}
    T^{\alpha\beta}_{\ \mu\nu}\equiv \frac{2\Lambda}{D\left(D-2\right)}\left(e^{\alpha\beta}e_{\mu\nu}-D\delta^{\alpha}_{\ \mu}\delta^{\beta}_{\ \nu}\right)\ ,
\end{equation}
the above equation can be generally solved by
\begin{equation}
    h_{\mu\nu}\left(\lambda\right)=\exp{\left(\lambda T\right)}^{\alpha\beta}_{\ \mu\nu}h_{\alpha\beta}\left(0\right)\ ,
\end{equation}
where:
\begin{equation}
    \exp{\left(\lambda T\right)}^{\alpha\beta}_{\ \mu\nu}=\delta^{\alpha}_{\ \mu}\delta^{\beta}_{\ \nu}+\lambda T^{\alpha\beta}_{\ \mu\nu}+ \frac{\lambda^2}{2}T^{\alpha\beta}_{\ \gamma\delta}T^{\gamma\delta}_{\ \mu\nu}+\dots
\end{equation}
\subsection{Bubble solution in AdS}
Let $\mathcal{M}$ be a $D$-dimensional non-compact manifold, endowed with coordinates $\left(t,u,x^\mu\right)$ and with a \textit{Euclidean} metric tensor $g_{\mu\nu}$. In particular, let's consider two values $u_0$ and $u_1$ of the radial coordinate, with $u_0<u_1$, such that:
\begin{enumerate}
    \item For $0<u<u_0$, the metric is that of Euclidean anti de Sitter space-time with cosmological constant $\Lambda_0$;
    \item For $r_0<u<u_1$, the metric is that of a domain wall interpolating among two values $\Lambda_0$ and $\Lambda_1$ of the cosmological constant;
    \item For $u>u_1$, the metric is that of Euclidean anti de Sitter space-time with cosmological constant $\Lambda_1$.
\end{enumerate}
We introduce two positive parameters
\begin{equation}
    2\varepsilon\equiv u_1-u_0\ ,\quad \varrho\equiv\frac{u_1+u_0}{2}\ ,
\end{equation}
respectively referring to the size and the centre of the domain wall.
Furthermore, we introduce $x\equiv u-\varrho$ and set $D=4$ for the sake of simplicity. Hence, we work with a metric tensor of the form
\begin{equation}
    \ds^{2}=\alpha^2\left(x\right)\left[\frac{\dx^2}{\left(x+\varrho\right)^2}+\left(x+\varrho\right)^2\dx^\mu\dx_\mu\right]\ ,
\end{equation}
where
\begin{equation}
    \alpha^2(x)\equiv\begin{cases}
        \begin{split}
        \alpha^2_{0}&\text{ for }x\leq-\varepsilon\\
        G(x)&\text{ for }-\varepsilon\leq x\leq\rho\\
        \alpha^2_{1}&\text{ for }x\geq\varepsilon
        \end{split}
    \end{cases}\ ,
\end{equation}
and the interpolating function is:
\begin{equation}
    G(x)\equiv\frac{\alpha^2_{1}+\alpha^2_{0}}{2}+\frac{\alpha^2_{1}-\alpha^2_{0}}{2}\tanh{\frac{x}{\left(\varepsilon-x\right)\left(x+\varepsilon\right)}}\ .
\end{equation}





\newpage
\begin{appendices}
\section{Ricci Tensor for product manifold}
Let $\mathcal{G}\equiv\mathcal{M}\times\mathcal{N}$ be a $\left(D_1+D_2\right)$-dimensional Euclidean product manifold, charted by local coordinates $z^M\equiv\left(x^{a},y^{\mu}\right)$, where $x^1,\dots,x^{D_1}$ parametrize $\mathcal{M}$ and $y^1,\dots,y^{D_2}$ parametrize $\mathcal{N}$. Let
\begin{equation}
    G_{MN}\left(x,y\right) =\begin{pmatrix}
   h_{ab}\left(x\right) & 0\\\
0 & g_{\mu\nu}\left(x,y\right) 
 \end{pmatrix}
\end{equation}
be a block-defined metric tensor on $\mathcal{G}$, where the metric components in directions tangential to $\mathcal{N}$ are allowed to depend on the coordinates of $\mathcal{M}$. At this point, we want to compute the Ricci tensor associated to $G_{MN}$. It the following, we put a \textit{tilde} on geometric quantities equally to those that would have been computed on $\mathcal{M}$ or $\mathcal{N}$ alone. First of all, we consider Christoffel symbols:
\begin{equation}
\begin{split}
    \Gamma^{a}_{bc}&=\frac{1}{2}h^{ad}\left(h_{bd,c}+h_{dc,b}-h_{cb,d}\right)=\Tilde{\Gamma}^{a}_{bc}\ ,\\
    \Gamma^{\mu}_{bc}&=0\ ,\quad \Gamma^{\mu}_{\nu c}=\frac{1}{2}g^{\mu\rho}g_{\nu\rho,c}\ ,\quad \Gamma^{a}_{\mu c}=0\ ,\quad \Gamma^{a}_{\mu\nu}=-\frac{1}{2}h^{ad}g_{\mu\nu,d}\ ,\\
    \Gamma^{\mu}_{\nu\sigma}&=\frac{1}{2}g^{\mu\rho}\left(g_{\nu\rho,\sigma}+g_{\sigma\rho,\nu}-g_{\nu\sigma,\rho}\right)=\Tilde{\Gamma}^{\mu}_{\nu\sigma}\ .
\end{split}
\end{equation}
Now, we can start computing the various components on the Ricci tensor. We obtain:
\begin{equation}
    \begin{split}
        R_{\mu\nu}&=R^{\rho}_{\ \mu\rho\nu}+R^{a}_{\ \mu a\nu}=  \partial_{\rho}\Gamma^{\rho}{}_{\nu\mu} -
  \partial_{\nu}\Gamma^{\rho}{}_{\rho\mu} +
  \Gamma^{\rho}{}_{\rho M}\Gamma^{M}{}_{\nu\mu} -\\
  &\quad +\Gamma^{\rho}{}_{\nu M}\Gamma^{M}{}_{\rho\mu}+\partial_{a}\Gamma^{a}{}_{\nu\mu} -
  \partial_{\nu}\Gamma^{a}{}_{a\mu} +
  \Gamma^{a}{}_{a M}\Gamma^{M}{}_{\nu\mu} -
  \Gamma^{a}{}_{\nu M}\Gamma^{M}{}_{a\mu}=\\
  &=\partial_{\rho}\Gamma^{\rho}{}_{\nu\mu} -
  \partial_{\nu}\Gamma^{\rho}{}_{\rho\mu} +
  \Gamma^{\rho}{}_{\rho \sigma}\Gamma^{\sigma}{}_{\nu\mu}+
  \Gamma^{\rho}{}_{\rho b}\Gamma^{b}{}_{\nu\mu} +\\
  &\quad -\Gamma^{\rho}{}_{\nu b}\Gamma^{b}{}_{\rho\mu}-\Gamma^{\rho}{}_{\nu \sigma}\Gamma^{\sigma}{}_{\rho\mu}+\partial_{a}\Gamma^{a}{}_{\nu\mu} -
  \partial_{\nu}\Gamma^{a}{}_{a\mu} +\\
  &\quad +\Gamma^{a}{}_{a b}\Gamma^{b}{}_{\nu\mu}+\Gamma^{a}{}_{a \sigma}\Gamma^{\sigma}{}_{\nu\mu} -
  \Gamma^{a}{}_{\nu b}\Gamma^{b}{}_{a\mu}-  \Gamma^{a}{}_{\nu \sigma}\Gamma^{\sigma}{}_{a\mu}=\\
  &=\Tilde{R}_{\mu\nu}+
  \Gamma^{\rho}{}_{\rho b}\Gamma^{b}{}_{\nu\mu} -\Gamma^{\rho}{}_{\nu b}\Gamma^{b}{}_{\rho\mu}-\partial_{a}\Gamma^{a}{}_{\nu\mu} +\Gamma^{a}{}_{a b}\Gamma^{b}{}_{\nu\mu} -  \Gamma^{a}{}_{\nu \sigma}\Gamma^{\sigma}{}_{a\mu}=\\
  &=\Tilde{R}_{\mu\nu}-\frac{1}{4}g^{\rho\sigma}h^{ab}g_{\rho\sigma,a}g_{\mu\nu,b} +\frac{1}{2}g^{\rho\sigma}h^{ab}g_{\nu\sigma,a}g_{\mu\rho,b}+\frac{1}{2}\de_a\left(h^{ab}g_{\mu\nu,b}\right)-\frac{1}{2}\Tilde{\Gamma}^{a}_{\ ab}h^{bc}g_{\mu\nu,c}\ .
    \end{split}
\end{equation}
Furthermore, we have:
\begin{equation}
      R^{\rho}{}_{\sigma\mu\nu} =
  \partial_{\mu}\Gamma^{\rho}{}_{\nu\sigma} -
  \partial_{\nu}\Gamma^{\rho}{}_{\mu\sigma} +
  \Gamma^{\rho}{}_{\mu\lambda}\Gamma^{\lambda}{}_{\nu\sigma} -
  \Gamma^{\rho}{}_{\nu\lambda}\Gamma^{\lambda}{}_{\mu\sigma}
\end{equation}
\end{appendices}

==> massive.tex <==
\subsection{Massive Perelman's Flow}
We now focus on the specific example of the flow equation induced by the action of a massive scalar field with no other coupling, on a space-time background admitting a cosmological constant. Namely, we take \eqref{aact} with:
\begin{equation}
    \left(g_{0},g_{1},g_{2},g_{3},\dots\right)\equiv\left(\Lambda,0,m^{2},0,\dots\right)
\end{equation}
Therefore, we get:
\begin{equation}
\begin{split}
    s_{\ k<2}^{(D)}=&\frac{\Lambda}{k!}\left(\frac{2}{2-D}\right)^{k}\ , \\
   s_{\ k\geq 2}^{(D)}=&\frac{\Lambda}{k!}\left(\frac{2}{2-D}\right)^{k}+\frac{m^{2}}{\left(k-2\right)!}\left(\frac{2}{2-D}\right)^{k-2}\frac{2D-3}{D-2}\ .
\end{split}
\end{equation}
By plugging the above expression into \eqref{acteq}, we get the desired flow equations at an arbitrary number of space-time dimensions.
\subsubsection{Einstein manifolds with constant scalar}
In order to write Massive Perelman's Flow down in a simple setting, we consider the case of a \textit{constant} scalar $\phi$ on an Einstein manifold background, with cosmological constant fixed by $g_{0}=\Lambda$. Therefore, we have:
\begin{equation}
    R_{\mu\nu}=\frac{R}{D}g_{\mu\nu}\ ,\quad R=D\Lambda\ .
\end{equation}
Hence, the flow equations reduce to:
\begin{equation}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)}\phi^{n-1}+\mathcal{L}_{\xi}g_{\mu\nu}\ ,\\
        \frac{\de\phi}{\de\lambda}=&-R-\frac{D}{2}\sum_{n=1}^{+\infty}ns_{\ n}^{(D)} \phi^{n-1}+\mathcal{L}_{\xi}\phi\ .
    \end{split}
\end{equation}
We define
\begin{equation}
    \begin{split}
        \Phi\equiv\sum_{k=1}^{+\infty}ks_{\ k}^{(D)}\phi^{k-1}
    \end{split}
\end{equation}
Thus, by neglecting the diffeomorphisms, we have:
\begin{equation}
        \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}\Phi\ ,\\
        \frac{\de \phi}{\de\lambda}=&-R-\frac{D}{2}\Phi\ .
    \end{split}
\end{equation}
By recasting the first equation in terms of the scalar curvature, we have:
\begin{equation}
\frac{\de R}{\de\lambda}=\frac{2R}{D}\left(R+\frac{D}{2}\Phi\right)\ .
\end{equation}
Hence, by defining
\begin{equation}
    \mathcal{A}\left(R,\phi\right)\equiv R+\frac{D}{2}\Phi\ ,
\end{equation}
we can solve for:
\begin{equation}
        \begin{split}
            \frac{\de R}{\de\lambda}=&\frac{2R}{D}\mathcal{A}\left(R,\phi\right)\ ,\\
        \frac{\de \phi}{\de\lambda}=&-\mathcal{A}\left(R,\phi\right)\ .
    \end{split}
\end{equation}
The only scales of the problem are those set by $m$ and $\Lambda$ and physics can be fully expressed by their ratio. Therefore, we can set $m=1$ and study the flow behaviour of $\Lambda$, via $R$, and $\phi$ without loss of generality.
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Gr.png}
    \caption{The blue region corresponds to $\mathcal{A}>0$, with $D=4$. The arrows correspond to the flow direction. The horizontal axis is labelled by $R=\Lambda/4$, while the vertical one by $\phi$ (we called it $f$, in order to distinguish the $D=4$ case from the general one.)}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=\linewidth]{Ff.png}
    \caption{Plot of $\Phi$ with respect to $\phi$, at $m=1$, for different values of the dimension $D$, taken between $3$ and $8$.It can be observed that the qualitative behaviour doesn't change between different values of $D$}
    \end{figure}
From the above picture it is clear that the $\mathcal{A}=0$ line, separating the blue and the white regions, can either be a stable or an unstable fixed point. In particular, fixed points can only exist for $R>R_{0}$, for some negative $R_{0}$. Indeed, fixed points form two branches between $R_{0}$ and some upper value $R_{1}$, beyond which we only have the lower branch:
\begin{itemize}
    \item The higher branch, with bigger values of $f$, is unstable;
    \item The lower branch, with smaller values of $f$, is stable.
\end{itemize}
Moreover, a further unstable branch appears for $\Bar{R}<R<R_{1}$, with $\Bar{R}$ falling between $R_{0}$ and $R_{1}$. 
In order to better analyse the system, we perform a diffeomorphism
\begin{equation}
        \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}\Phi+\mathcal{L}_{\chi}g_{\mu\nu}=\\
        =&-2\frac{R}{D} g_{\mu\nu}-g_{\mu\nu}\Phi+\nabla_{\mu}\chi_{\nu}+\nabla_{\nu}\chi_{\mu}\ ,\\
        \frac{\de \phi}{\de\lambda}=&-R-\frac{D}{2}\Phi+\mathcal{L}_{\chi}\phi=\\
        =&-R-\frac{D}{2}\Phi+\chi^{\mu}\de_{\mu}\phi\ ,
    \end{split}
\end{equation}
sourced by a vector field $\chi^{\mu}$. In particular, we impose:
\begin{equation}
    \nabla_{\mu}\chi_{\nu}+\nabla_{\nu}\chi_{\mu}=g_{\mu\nu}\Phi\ .
\end{equation}
By contracting with the inverse metric, we get:
\begin{equation}
    \nabla_{\mu}\chi^{\mu}=\frac{D}{2}\Phi\ .
\end{equation}
Expanding the two sides, we see that $\chi$ depends on the flow-dependent metric and scalar in a highly non-trivial way:
\begin{equation}
    \partial_{\mu}\chi^{\mu}+\frac{1}{2}g^{\mu\alpha}\chi^{\nu}\partial_{\nu}g_{\alpha\mu}=\frac{D}{2}\Phi
\end{equation}
By defining
\begin{equation}
    \begin{split}
    A_{\nu}&\equiv -\frac{1}{2}g^{\mu\alpha}\partial_{\nu}g_{\alpha\mu}\ ,\\
        B&\equiv \frac{D}{2}\Phi\ ,
    \end{split}
\end{equation}
we get:
\begin{equation}
    \partial_{\mu}\chi^{\mu}\left(x\right)=A_{\mu}\left(x\right)\chi^{\mu}\left(x\right)+B\ .
\end{equation}
Since the flow fully translates in an evolution in $\Lambda$ and $\phi$, we are sure that the metric can be written as
\begin{equation}
    g=diag\left(-G(r),G(r)^{-1},r^{2},r^{2}\sin^{2}{\vartheta}\right)\ ,
\end{equation}
in spherical coordinates for any value of the flow parameter $\lambda$. Hence, we exploit the following anstaz:
\begin{equation}
    \chi^{\mu}=\delta^{\mu}_{r}\rho(r)\ .
\end{equation}
Hence, the equation for the vector field components reduces to
\begin{equation}
    \rho'(r)=\frac{4}{r}\rho(r)+B\ ,
\end{equation}
which can be solved as:
\begin{equation}
    \rho(r)=-\frac{D\Phi}{6}r\ .
\end{equation}
Therefore, under the diffeomorphism we get:
\begin{equation}
           \begin{split}
        \frac{\de R}{\de\lambda}=&\frac{2R^{2}}{D}\ ,\\
        \frac{\de \phi}{\de\lambda}=&-R-\frac{D}{2}\Phi-\frac{D\Phi}{6}r\de_{r}\phi\ .
    \end{split} 
\end{equation}
Now the flow equation for the scalar curvature is decoupled from the scalar evolution and can be simply solved as:
\begin{equation}
    R\left(\lambda\right)=\frac{DR_{0}}{D-2R_{0}\lambda}\ .
\end{equation}
Furthermore, being the scalar constant, the diffomorphism-dependent term drops from its flow equation. Hence, we only have to solve for:
\begin{equation}
    \frac{\de \phi}{\de\lambda}=\frac{DR_{0}}{2R_{0}\lambda-D}-\frac{D}{2}\Phi\ .
\end{equation}
The only thing we are left to do is computing $\Phi$ explicitly, so that the flow equation for $\phi$ can be solved. We have, for $m=1$:
\begin{equation}
\begin{split}
    \Phi=& \sum_{k=1}^{+\infty}ks_{\ k}^{(D)}\phi^{k-1}= \sum_{k=1}^{+\infty}k\frac{\Lambda}{k!}\left(\frac{2}{2-D}\right)^{k}\phi^{k-1}+\\
    &+\sum_{k=2}^{+\infty}k\frac{1}{\left(k-2\right)!}\left(\frac{2}{2-D}\right)^{k-2}\frac{2D-3}{D-2}\phi^{k-1}=\\
    =& \Lambda\left(\frac{2}{2-D}\right)\exp{\left(\frac{2\phi}{2-D}\right)}+\frac{2D-3}{D-2}\phi\sum_{k=0}^{+\infty}\frac{k+2}{k!}\left(\frac{2}{2-D}\right)^{k}\phi^{k}=\\
    =& \Lambda\left(\frac{2}{2-D}\right)\exp{\left(\frac{2\phi}{2-D}\right)}+\frac{4D-6}{D-2}\phi\exp{\left(\frac{2\phi}{2-D}\right)}+\\
&+\frac{2D-3}{D-2}\phi^{2}\sum_{k=0}^{+\infty}\frac{k}{k!}\left(\frac{2}{2-D}\right)^{k}\phi^{k-1}=\\
=& \Lambda\left(\frac{2}{2-D}\right)\exp{\left(\frac{2\phi}{2-D}\right)}+\frac{4D-6}{D-2}\phi\exp{\left(\frac{2\phi}{2-D}\right)}+\\
&+\frac{2D-3}{D-2}\phi^{2}\frac{\de}{\de\phi}\exp{\left(\frac{2\phi}{2-D}\right)}=\\
=&\frac{2D-3}{D-2}\left(\phi^{2}\frac{\de}{\de\phi}+2\phi+\frac{2\Lambda}{3-2D}\right)\exp{\left(\frac{2\phi}{2-D}\right)}
\end{split}
\end{equation}
Remembering that the $\Lambda$ factor appearing in $\Phi$ is a flowing quantity, with
\begin{equation}
    \Lambda\left(\lambda\right)=\frac{R\left(\lambda\right)}{D}=\frac{R_{0}}{D-2R_{0}\lambda}\ ,
\end{equation}
we can plug the above formula into the flow equation for $\phi$ and solve it numerically. In particular, for $D=4$, we have:
\begin{equation}
    \frac{\de \phi}{\de\lambda}=\frac{4\Lambda_{0}}{2\Lambda_{0}\lambda-1}-\left(10\phi-5\phi^{2}-\frac{2\Lambda_{0}}{2\Lambda_{0}\lambda-1}\right)e^{-\phi}\ .
\end{equation}
In order to properly solve the above equation via numerical methods, we must consider a few cases separately.
\paragraph{Zero cosmological constant}
By taking the simplest possible scenario, namely $\Lambda_{0}=0$, we reduce to study the massive Perelman evolution equation
\begin{equation}
    \frac{\de \phi}{\de\lambda}=5\left(\phi^{2}-2\phi\right)e^{-\phi}\ ,
\end{equation}
for a scalar field in Minkowski space-time.
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Graph1.png}
    \caption{Massive Perelman flow of a constant scalar field on $4D$ Minkowski background, with initial value $\phi_{0}=1$.}
    \label{graph1}
\end{figure}
\paragraph{Positive cosmological constant}
Concerning the case of a positive cosmological constant $\Lambda_{0}>0$, thing get less trivial. Indeed, the flow reaches a finite time singularity at
\begin{equation}
    \lambda_{\infty}=\frac{1}{2\Lambda_{0}}\ ,
\end{equation}
when $\Lambda(\lambda)$ blows to infinity. Therefore, it is interesting to investigate what happens to $\phi$ at the singularity. Numerically, it can be shown that this strongly depends on the initial value for $\phi$.
\paragraph{Negative cosmological constant}
Regarding, on the hand, the case of a negative cosmological constant, we have no singularity and the metric asymptotically approaches Minkowski space-time. Therefore, the flow can be properly approximated by the evolution depicted in Figure \ref{graph1}. Concerning what happens before $\Lambda$ gets negligible, we observe, for positive $\phi_{0}$, the appearance of a minimum.
    \begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Graph2.png}
    \caption{Massive Perelman flow of a constant scalar field on $4D$ Anti de Sitter background, with initial value $\phi_{0}=1$ and cosmological constant evolving according to Ricci flow from $\Lambda_{0}=-5$ to $0$.}
    \label{graph1}
\end{figure}

==> name.tex <==
Therefore, we can straightforwardly observe that, for Anti de Sitter space-time, the cosmological constant does nothing more than enhancing the contribution of $\chi$, particularly for early flow times and large values of $\rho$. Hence, there's no qualitative difference with the analysis developed in section \ref{Minkowski}. Since $\Lambda\rightarrow 0$, even the asymptotic radius of shrinking bubbles in the $\chi<0$ regime is unchanged from the previous discussion.
\subsection{de Sitter background}
Once more, we find ourselves with the thin-wall regime flow equation:
\begin{equation}
       \Dot{\varrho}=\frac{3}{\varrho}+\chi\left(1-\frac{\Lambda\varrho^2}{3}\right)\ .
\end{equation}


\section{Minkowski with a non-trivial dilatonic bubble}
Starting from the flow equations \eqref{form2}, we construct a slightly less trivial setting with respect to the one considered in section \ref{Minkowski}. We assume, as before, the metric to be that of flat $4$-dimensional Minkowski for any value of $r$. On top of that, we consider a sphere around the origin with radius $\varrho$ and assume the dilaton, far enough from its boundary, to take the two expressions
\begin{equation}
    f_{a}\left(r\right)\equiv f_{1}-\frac{2}{r}\quad\text{   and   }\quad   f_{b}\left(r\right)\equiv f_{2}-\frac{2}{r},
\end{equation}
with $f_{1}\neq f_{2}$, inside and outside the sphere respectively. We can easily observe that It is clear that, in order to study the $4$-dimensional metric, we must re-define the fields via a Weyl rescaling and recover Einstein-Hilbert action as a first term in the low energy action. We know that, by imposing
\begin{equation}
    \Tilde{g}_{\mu\nu}\equiv e^{2\omega}g_{\mu\nu}\ ,
\end{equation}
we have
\begin{equation}
    \sqrt{-\Tilde{g}}=\sqrt{-g}e^{4\omega}
\end{equation}
and
\begin{equation}
    R_{\Tilde{g}}=e^{-2\omega}R_{g}-6e^{-2\omega}\Delta\omega-6e^{-2\omega}\de^{\mu}\omega\de_{\mu}\omega\ .
\end{equation}
Hence, we obtain:
\begin{equation}
            S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{4}}\diff^{4}x\sqrt{-g}e^{2\omega}e^{3\sigma}\left(R_{g}-6\Delta\omega-6\de^{\mu}\omega\de_{\mu}\omega-\frac{21}{2}e^{2\omega}\de^{\mu}\sigma\de_{\mu}\sigma\right)\ .
\end{equation}
By picking
\begin{equation}
    \omega\equiv-\frac{3}{2}\sigma\ ,
\end{equation}
the above reduces to:
\begin{equation}
            S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{4}}\diff^{4}x\sqrt{-g}\left(R_{g}+9\Delta\sigma-9\de^{\mu}\sigma\de_{\mu}\sigma-\frac{21}{2}e^{-3\sigma}\de^{\mu}\sigma\de_{\mu}\sigma\right)\ .
\end{equation}
Being $\tau\equiv 3\sigma$, we have:
\begin{equation}
            S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{4}}\diff^{4}x\sqrt{-g}\left[R_{g}+\Delta\tau-\left(1+\frac{3}{2}e^{-\tau}\right)\de^{\mu}\tau\de_{\mu}\tau\right]\ .
\end{equation}
Getting rid of the boundary term $\sim\Delta\tau$, we obtain:
\begin{equation}
            S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{4}}\diff^{4}x\sqrt{-g}\left[R_{g}-\left(1+\frac{3}{2}e^{-\tau}\right)\de^{\mu}\tau\de_{\mu}\tau\right]\ .
\end{equation}

\section{Metric-Modulus Flow}
\subsection{Dimensional Reduction}
Now, we want to define an alternative set of flow equations, for a $4$-dimensional setting comprising a Lorentzian metric $g_{\mu\nu}$ and a scalar modulus $\tau$, emerging as a radius parameter for some compact dimensions. In order to so so, we consider $10$-dimensional Einstein-Hilbert action
\begin{equation}
    S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{10}}\diff^{10}x\sqrt{-G}R_{G}\ ,
\end{equation}
where $G_{MN}$ is the $10$-dimensional metric on $\mathcal{M}_{10}$, and perform a peculiar $T^{6}$ compactification. In order to do so, we impose 
\begin{equation}
    \mathcal{M}_{10}=\mathcal{M}_{4}\times T^6\ ,
\end{equation}
for which the metric decomposes as follows
\begin{equation}
    G_{MN}=\left(
\begin{array}{c|c}
g_{\mu\nu}  & 0 \\ \hline
 0 & h_{mn}
\end{array}\right)\ ,
\end{equation}
where $h_{mn}$ is the metric
\begin{equation}\label{metric}
    h_{mn}=e^{\sigma}\delta_{mn}
\end{equation}
for a $T^6$ where all the radii are set to be equal to $e^{\sigma}$. By splitting the $10$-dimensional charts as $\left(x^{\mu},y^{m}\right)$, where the $x^{\mu}$ cover $\mathcal{M}_{4}$ and the $y^m$ cover $T^6$, we assume $\sigma=\sigma\left(x^{\mu}\right)$. Namely, we take the modulus not to depend on internal coordinates. By plugging \eqref{metric} into the definition of $R_{G}$, we get:
\begin{equation}
    R_{G}=R_{g}-\frac{21}{2}\nabla^{\mu}\sigma\nabla_{\mu}\sigma-6\nabla^{2}\sigma\ .
\end{equation}
Furthermore, we have:
\begin{equation}
    \sqrt{-G}=\sqrt{-g}e^{3\sigma}\ .
\end{equation}
Thus, we are left with the lower dimensional effective action:
\begin{equation}
        S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{4}}\diff^{4}x\sqrt{-g}e^{3\sigma}\left(R_{g}-\frac{21}{2}\nabla^{\mu}\sigma\nabla_{\mu}\sigma-6\nabla^{2}\sigma\right)\ .
\end{equation}
By defining $\tau\equiv-3\sigma$, we obtain:
\begin{equation}\label{modul}
        S=\frac{1}{2\kappa_{10}^2}\int_{\mathcal{M}_{4}}\diff^{4}x\sqrt{-g}\left[R_{g}-\frac{7}{6}\left(\nabla\tau\right)^2+2\nabla^{2}\tau\right]e^{-\tau}\ .
\end{equation}
\subsection{Flow equations}
In the following discussion, we move to a more general setting and derive the geometric flow equations associated to the \textit{euclidean} entropy functional 
\begin{equation}\label{funk}
        \mathcal{F}_{\left(\alpha,\beta,\gamma\right)}\left(g,\phi\right)=\int\diff^{D}x\sqrt{g}e^{-\phi}\left[R+\alpha\left(\nabla\phi\right)^2+\beta\phi^2+\gamma\nabla^{2}\phi\right]\ .
\end{equation}
for a rank-$2$ symmetric tensor $g_{\mu\nu}$ and a scalar $\phi$, where an extra quadratic term for $\phi$ was included for generality and the proportionality constant, which can always be reabsorbed in the flow parameter, was set to $1$. The standard metric-dilaton flow equations \eqref{form2} correspond to the $\left(\alpha,\beta,\gamma\right)=\left(1,0,0\right)$ case, while the metric-modulus flow associated to \eqref{modul} corresponds to $\left(\alpha,\beta,\gamma\right)=\left(-7/2,0,0\right)$. It must be noted that the $k$ parameter measures the significance of domain walls for $\phi$, as is usually done in Ginzburg-Landau theory. In order to derive the flow equations, we perform variations in $\phi$ and $g_{\mu\nu}$ so that:
\begin{equation}
    \delta\left(\sqrt{g}e^{-\phi}\right)=0\ .
\end{equation}
By taking the first order variation
\begin{equation}
    \begin{split}
        g_{\mu\nu}&\longmapsto g_{\mu\nu}+v_{\mu\nu}\\
        g^{\mu\nu}&\longmapsto g^{\mu\nu}-v^{\mu\nu}\\
        \phi&\longmapsto\phi+h\ ,
    \end{split}
\end{equation}
we have the following
\begin{equation}
\begin{split}
    \delta\left(\nabla\phi\right)^2&=\nabla^{\mu}\phi\nabla^{\nu}\phi v_{\mu\nu}+2g_{\mu\nu}\nabla^{\mu}\phi\nabla^{\nu}h\\
    \delta\nabla^{2}\phi&=-v^{\mu\nu}\nabla_{\mu}\nabla_{\nu}\phi-\delta\Gamma^{\lambda}_{\mu\nu}\nabla_{\lambda}\phi+\nabla^{2}h=\\
    &=-v^{\mu\nu}\nabla_{\mu}\nabla_{\nu}\phi-\frac{1}{2}\left(\nabla_{\mu}v_{\nu\xi}+\nabla_{\nu}v_{\mu\xi}-\nabla_{\xi}v_{\nu\mu}\right)\nabla^{\xi}\phi+\nabla^{2}h\\
    \delta R&=-\nabla^{2}v+\nabla^{\mu}\nabla^{\nu}v_{\mu\nu}-R_{\mu\nu} v^{\mu\nu}\\
    \delta\phi^2&=2\phi h\ .
\end{split}
\end{equation}
where $v\equiv g^{\mu\nu}v_{\mu\nu}$.
At this point, we analyse all the functional terms separately, singling the fields variations out. Starting from the quadratic term, we simply have:
\begin{equation}
    \delta\int\diff^{D}x\sqrt{g}e^{-\phi}\beta\phi^2=\int\diff^{D}x\sqrt{g}e^{-\phi}2\beta\phi h\ .
\end{equation}
Studying the kinetic term for the scalar and getting rid of boundary terms, we obtain:
\begin{equation}
\begin{split}
    \delta\int\diff^{D}x\sqrt{g}e^{-\phi}\alpha\left(\nabla\phi\right)^2=&-\int\diff^{D}x\sqrt{g}e^{-\phi}\alpha\nabla_{\mu}\phi\nabla_{\nu}\phi v^{\mu\nu}+\\
    &+\int\diff^{D}x\sqrt{g}e^{-\phi}2\alpha \nabla_{\mu}\phi\nabla^{\mu}h=\\
    =&-\int\diff^{D}x\sqrt{g}e^{-\phi}\alpha\nabla_{\mu}\phi\nabla_{\nu}\phi v^{\mu\nu}+\\
    &+\int\diff^{D}x\sqrt{g}e^{-\phi}2\alpha \left[\left(\nabla\phi\right)^2-\nabla^{2}\phi\right]h
\end{split}
\end{equation}
Now, we move to the curvature term and, removing boundary terms, get:
\begin{equation}
    \begin{split}
        \delta\int\diff^{D}x\sqrt{g}e^{-\phi}R=&-\int\diff^{D}x\sqrt{g}e^{-\phi}R_{\mu\nu}v^{\mu\nu}-\int\diff^{D}x\sqrt{g}e^{-\phi}\nabla^{2}v+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\nabla^{\mu}\nabla^{\nu}v_{\mu\nu}=\\
        =&-\int\diff^{D}x\sqrt{g}e^{-\phi}R_{\mu\nu}v^{\mu\nu}-\int\diff^{D}x\sqrt{g}\nabla^{2}e^{-\phi}v+\\
        &+\int\diff^{D}x\sqrt{g}\nabla^{\nu}\nabla^{\mu}e^{-\phi}v_{\mu\nu}\ .
    \end{split}
\end{equation}
Before going on, we observe that:
\begin{equation}
    \nabla^{\nu}\nabla^{\mu}e^{-\phi}=e^{-\phi}\left(\nabla^{\nu}\phi\nabla^{\mu}\phi-\nabla^{\nu}\nabla^{\mu}\phi\right)\ .
\end{equation}
Hence, we are left with:
\begin{equation}
    \begin{split}
        \delta\int\diff^{D}x\sqrt{g}e^{-\phi}R=&-\int\diff^{D}x\sqrt{g}e^{-\phi}R_{\mu\nu}v^{\mu\nu}+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\left[\nabla^{2}\phi-\left(\nabla\phi\right)^2\right]v+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\left(\nabla^{\nu}\phi\nabla^{\mu}\phi-\nabla^{\nu}\nabla^{\mu}\phi\right)v_{\mu\nu}\ .
    \end{split}
\end{equation}
At this point, we study the two derivatives term:
\begin{equation}
    \begin{split}
        \delta\int\diff^{D}x\sqrt{g}e^{-\phi}\nabla^{2}\phi=&-\int\diff^{D}x\sqrt{g}e^{-\phi}v^{\mu\nu}\nabla_{\mu}\nabla_{\nu}\phi+\int\diff^{D}x\sqrt{g}e^{-\phi}\nabla^{2}h+\\
        &-\int\diff^{D}x\sqrt{g}e^{-\phi}\frac{1}{2}\left(\nabla_{\mu}v_{\nu\xi}+\nabla_{\nu}v_{\mu\xi}-\nabla_{\xi}v_{\nu\mu}\right)\nabla^{\xi}\phi=\\
        =&-\int\diff^{D}x\sqrt{g}e^{-\phi}v^{\mu\nu}\nabla_{\mu}\nabla_{\nu}\phi+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\left[\left(\nabla\phi\right)^{2}-\nabla^{2}\phi\right]h+\\
        &-\int\diff^{D}x\sqrt{g}e^{-\phi}\frac{1}{2}g^{\mu\nu}\left(\nabla_{\mu}v_{\nu\xi}+\nabla_{\nu}v_{\mu\xi}-\nabla_{\xi}v_{\nu\mu}\right)\nabla^{\xi}\phi\ .
    \end{split}
\end{equation}
Focusing on the last term, we have objects like
\begin{equation}
    \begin{split}
       \frac{1}{2}\int\diff^{D}x\sqrt{g}e^{-\phi}g^{\mu\nu}\nabla^{\xi}\phi\nabla_{\alpha}v_{\rho\eta}=&\frac{1}{2}\int\diff^{D}x\sqrt{g}g^{\mu\nu}\nabla_{\alpha}\left(e^{-\phi}\nabla^{\xi}\phi\right)v_{\rho\eta}=\\
       =&\frac{1}{2}\int\diff^{D}x\sqrt{g}e^{-\phi}g^{\mu\nu}\left(\nabla_{\alpha}\nabla^{\xi}\phi-\nabla_{\alpha}\phi\nabla^{\xi}\phi\right)v_{\rho\eta}
    \end{split}
\end{equation}
with different indices. Putting them together, we obtain:
\begin{equation}
    \begin{split}
        \delta\int\diff^{D}x\sqrt{g}e^{-\phi}\nabla^{2}\phi=&-\int\diff^{D}x\sqrt{g}e^{-\phi}v^{\mu\nu}\nabla_{\mu}\nabla_{\nu}\phi+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\left[\left(\nabla\phi\right)^{2}-\nabla^{2}\phi\right]h+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\frac{1}{2}\left[\nabla^{2}\phi-\left(\nabla\phi\right)^{2}\right]v+\\
        &-\int\diff^{D}x\sqrt{g}e^{-\phi}\left(\nabla_{\mu}\nabla_{\nu}\phi-\nabla_{\mu}\phi\nabla_{\nu}\phi\right)v^{\mu\nu}=\\
        =&\int\diff^{D}x\sqrt{g}e^{-\phi}\left[\left(\nabla\phi\right)^{2}-\nabla^{2}\phi\right]h+\\
        &+\int\diff^{D}x\sqrt{g}e^{-\phi}\frac{1}{2}\left[\nabla^{2}\phi-\left(\nabla\phi\right)^{2}\right]v+\\
        &-\int\diff^{D}x\sqrt{g}e^{-\phi}\left(2\nabla_{\mu}\nabla_{\nu}\phi-\nabla_{\mu}\phi\nabla_{\nu}\phi\right)v^{\mu\nu}
    \end{split}
\end{equation}
Now, we consider the variation of the functional and collect all the above terms. We have
\begin{equation}
    \begin{split}
        \delta\mathcal{F}_{\left(\alpha,\beta,\gamma\right)}\left(g,\phi\right)=&\int\diff^{D}x\sqrt{g}e^{-\phi}\biggl\{2\bigl[\beta\phi+\left(\alpha+\gamma\right)\left(\nabla\phi\right)^2-\left(\alpha+\gamma\right)\nabla^{2}\phi\bigr]h+\\
        &+\bigl[-R_{\mu\nu}+\left(1-\alpha+\gamma\right)\nabla_{\mu}\phi\nabla_{\nu}\phi-\left(1+2\gamma\right)\nabla_{\nu}\nabla_{\mu}\phi+\\
        &+\left(1+\frac{\gamma}{2}\right)g_{\mu\nu}\nabla^{2}\phi-\left(1+\frac{\gamma}{2}\right)g_{\mu\nu}\left(\nabla\phi\right)^2\bigr]v^{\mu\nu}\biggr\}\ .
    \end{split}
\end{equation}
Furthermore, we have
\begin{equation}\label{condition}
    \delta\left(\sqrt{g}e^{-\phi}\right)=0\Longrightarrow h=\frac{v}{2}\ .
\end{equation}
By plugging this result into the above expression, we get:
\begin{equation}
    \begin{split}
        \delta\mathcal{F}_{\left(\alpha,\beta\right)}\left(g,\phi\right)=&\int\diff^{D}x\sqrt{g}e^{-\phi}\biggl[-R_{\mu\nu}+\left(1-\alpha+\gamma\right)\nabla_{\mu}\phi\nabla_{\nu}\phi-\left(1+2\gamma\right)\nabla_{\nu}\nabla_{\mu}\phi+\\
        &+g_{\mu\nu}\beta\phi+\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\nabla^{2}\phi-\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\left(\nabla\phi\right)^2\biggr]v^{\mu\nu}\ .
    \end{split}
\end{equation}
Hence, we introduce a flow parameter $\lambda$ and set the flow equation for the metric to be:
\begin{equation}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}+g_{\mu\nu}2\beta\phi+2\left(1-\alpha+\gamma\right)\nabla_{\mu}\phi\nabla_{\nu}\phi-2\left(1+2\gamma\right)\nabla_{\nu}\nabla_{\mu}\phi+\\
        &+2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\nabla^{2}\phi-2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\left(\nabla\phi\right)^2\ .
    \end{split}
\end{equation}
From the condition derived in \eqref{condition}, we also get:
\begin{equation}
    \begin{split}
        \frac{\de\phi}{\de\lambda}=&-R+D\beta\phi+\left[\left(1-\alpha\right)\left(1-D\right)+\gamma\left(1+\frac{D}{2}\right)\right]\left(\nabla\phi\right)^{2}+\\
        &-\left[1-D\left(1-\alpha\right)+\gamma\left(2+\frac{D}{2}\right)\right]\nabla^{2}\phi\ .
    \end{split}
\end{equation}
It can be straightforwardly observed that, by taking $\left(\alpha,\beta,\gamma\right)=\left(1,0,0\right)$, we can get back the flow equations \eqref{form1}. By also introducing DeTurk's diffeomorphism, as the flow induced by some vector field $\xi^{\mu}$, we finally get the general $D$-dimensional gradient flow equations associated to the entropy functional \eqref{funk}:
\begin{equation}\label{geneq}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}+g_{\mu\nu}2\beta\phi+2\left(1-\alpha+\gamma\right)\nabla_{\mu}\phi\nabla_{\nu}\phi-2\left(1+2\gamma\right)\nabla_{\nu}\nabla_{\mu}\phi+\\
        &+2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\nabla^{2}\phi-2\left(1-\alpha-\frac{\gamma}{2}\right)g_{\mu\nu}\left(\nabla\phi\right)^2+\mathcal{L}_{\xi}g_{\mu\nu}\ ,\\
        \frac{\de\phi}{\de\lambda}=&-R+D\beta\phi+\left[\left(1-\alpha\right)\left(1-D\right)+\gamma\left(1+\frac{D}{2}\right)\right]\left(\nabla\phi\right)^{2}+\\
        &-\left[1-D\left(1-\alpha\right)+\gamma\left(2+\frac{D}{2}\right)\right]\nabla^{2}\phi+\mathcal{L}_{\xi}\phi\ .
    \end{split}
\end{equation}
Therefore, the flow equations associated to the reduced action 
\eqref{modul}, when regarded as an entropy functional, can be obtained from \eqref{geneq} by setting $\left(
\alpha,\beta,\gamma\right)=\left(-7/6,0,2\right)$ and $D=4$:
\begin{equation}
    \begin{split}
        \frac{\de g_{\mu\nu}}{\de\lambda}=&-2R_{\mu\nu}+\frac{25}{3}\nabla_{\mu}\phi\nabla_{\nu}\phi-10\nabla_{\nu}\nabla_{\mu}\phi+\frac{7}{3}g_{\mu\nu}\nabla^{2}\phi-\frac{7}{3}g_{\mu\nu}\left(\nabla\phi\right)^2+\mathcal{L}_{\xi}g_{\mu\nu}=\\
        \equiv&v_{\mu\nu}+\mathcal{L}_{\xi}g_{\mu\nu}\ ,\\
        \frac{\de\phi}{\de\lambda}=&-R-\frac{1}{2}\left(\nabla\phi\right)^{2}-\frac{1}{3}\nabla^{2}\phi+\mathcal{L}_{\xi}\phi=\\
        \equiv&h+\mathcal{L}_{\xi}\phi\ .
    \end{split}
\end{equation}
\section{Two scalar fields}
Now, we derive the gradient flow equations for a general theory comprised of two scalar fields. We start from the simplest possible cases, generalising then to more cumbersome scenarios.
\subsection{}
